ITS: Implicit Thin Shell for Polygonal Meshes

In computer graphics, simplifying a polygonal mesh surface~$\mathcal{M}$ into a geometric proxy that maintains close conformity to~$\mathcal{M}$ is crucial, as it can significantly reduce computational demands in various applications. In this paper, we introduce the Implicit Thin Shell~(ITS), a concept designed to implicitly represent the sandwich-walled space surrounding~$\mathcal{M}$, defined as~$\{\textbf{x}\in\mathbb{R}^3|\epsilon_1\leq f(\textbf{x}) \leq \epsilon_2, \epsilon_1< 0, \epsilon_2>0\}$. Here, $f$ is an approximation of the signed distance function~(SDF) of~$\mathcal{M}$, and we aim to minimize the thickness~$\epsilon_2-\epsilon_1$. To achieve a balance between mathematical simplicity and expressive capability in~$f$, we employ a tri-variate tensor-product B-spline to represent~$f$. This representation is coupled with adaptive knot grids that adapt to the inherent shape variations of~$\mathcal{M}$, while restricting~$f$'s basis functions to the first degree. In this manner, the analytical form of~$f$ can be rapidly determined by solving a sparse linear system. Moreover, the process of identifying the extreme values of~$f$ among the infinitely many points on~$\mathcal{M}$ can be simplified to seeking extremes among a finite set of candidate points. By exhausting the candidate points, we find the extreme values~$\epsilon_1<0$ and $\epsilon_2>0$ that minimize the thickness. The constructed ITS is guaranteed to wrap~$\mathcal{M}$ rigorously, without any intersections between the bounding surfaces and~$\mathcal{M}$. ITS offers numerous potential applications thanks to its rigorousness, tightness, expressiveness, and computational efficiency. We demonstrate the efficacy of ITS in rapid inside-outside tests and in mesh simplification through the control of global error.

==> tab.tex <==
\begin{table*}[th]
	\centering
	\caption{The thickness and time-consumption of some selected meshes from Thingi10k.}
	\label{tab:genus}
	\scalebox{0.85}{
	\begin{tabular}{lcc|ccccc|rrrrr}
		\hline
		\multicolumn{3}{c|}{Models from Thingi10k} & \multicolumn{5}{c|}{Thickness~($\times 10^{-2}$)} & \multicolumn{5}{c}{Consuming Time~(seconds)}\\
		\hline
		\multicolumn{1}{c}{File ID} & \multicolumn{1}{c}{$|\text{V}|$} & \multicolumn{1}{c|}{$|\text{F}|$} & \multicolumn{1}{c}{6} & \multicolumn{1}{c}{7}& \multicolumn{1}{c}{8} & \multicolumn{1}{c}{9}& \multicolumn{1}{c|}{10}& \multicolumn{1}{c}{6} & \multicolumn{1}{c}{7}& \multicolumn{1}{c}{8} & \multicolumn{1}{c}{9}& \multicolumn{1}{c}{10}\\
		\hline
		
		\multicolumn{1}{l}{313880} & \multicolumn{1}{l}{13525} & 
		\multicolumn{1}{l|}{27058} &
		\multicolumn{1}{c}{3.44} & \multicolumn{1}{c}{1.62}& \multicolumn{1}{c}{0.91} & \multicolumn{1}{c}{0.43}& \multicolumn{1}{c|}{0.23}
		& \multicolumn{1}{r}{4.712} & \multicolumn{1}{r}{4.967}& \multicolumn{1}{r}{7.309} & \multicolumn{1}{r}{12.485}&\multicolumn{1}{r}{28.417}\\
		
		\multicolumn{1}{l}{37731} & \multicolumn{1}{l}{5480} & 
		\multicolumn{1}{l|}{11084} &
		\multicolumn{1}{c}{3.61} & \multicolumn{1}{c}{1.65}& \multicolumn{1}{c}{0.86} & \multicolumn{1}{c}{0.42}&\multicolumn{1}{c|}{0.23}
		& \multicolumn{1}{r}{2.226} & \multicolumn{1}{r}{2.361}& \multicolumn{1}{r}{3.886} & \multicolumn{1}{r}{10.142}&\multicolumn{1}{r}{36.132}\\
  
            \multicolumn{1}{l}{131971} & \multicolumn{1}{l}{16323} & \multicolumn{1}{l|}{32794} &
		\multicolumn{1}{c}{3.25} & \multicolumn{1}{c}{1.39}& \multicolumn{1}{c}{0.70} & \multicolumn{1}{c}{0.38}&\multicolumn{1}{c|}{0.20 }
		& \multicolumn{1}{r}{6.613} & \multicolumn{1}{r}{8.160}& \multicolumn{1}{r}{12.064} & \multicolumn{1}{r}{24.360}&\multicolumn{1}{r}{69.920}\\
    
		\multicolumn{1}{l}{80352} & \multicolumn{1}{l}{10630} & \multicolumn{1}{l|}{22512} &
		\multicolumn{1}{c}{3.54} & \multicolumn{1}{c}{1.87}& \multicolumn{1}{c}{0.88} & \multicolumn{1}{c}{0.49}&\multicolumn{1}{c|}{0.27}
		& \multicolumn{1}{r}{4.179} & \multicolumn{1}{r}{5.034}& \multicolumn{1}{r}{10.625} & \multicolumn{1}{r}{28.098}&\multicolumn{1}{r}{102.365}\\

        \multicolumn{1}{l}{32770} & \multicolumn{1}{l}{18944} & \multicolumn{1}{l|}{37884} &
		\multicolumn{1}{c}{3.11} & \multicolumn{1}{c}{1.80}& \multicolumn{1}{c}{0.85} & \multicolumn{1}{c}{0.42}&\multicolumn{1}{c|}{0.20}
		& \multicolumn{1}{r}{6.537} & \multicolumn{1}{r}{8.007}& \multicolumn{1}{r}{10.083} & \multicolumn{1}{r}{13.839}&\multicolumn{1}{r}{26.167}\\

        \multicolumn{1}{l}{47984} & \multicolumn{1}{l}{140864} & \multicolumn{1}{l|}{281724} &
		\multicolumn{1}{c}{3.01} & \multicolumn{1}{c}{1.50}& \multicolumn{1}{c}{0.79} & \multicolumn{1}{c}{0.44}&\multicolumn{1}{c|}{0.20}
		& \multicolumn{1}{r}{56.194} & \multicolumn{1}{r}{62.748}& \multicolumn{1}{r}{66.252} & \multicolumn{1}{r}{73.213}&\multicolumn{1}{r}{104.945}\\
        
        \multicolumn{1}{l}{48124} & \multicolumn{1}{l}{38788} & \multicolumn{1}{l|}{78336} &
		\multicolumn{1}{c}{2.65} & \multicolumn{1}{c}{1.51}& \multicolumn{1}{c}{0.66} & \multicolumn{1}{c}{0.30}&\multicolumn{1}{c|}{0.14}
		& \multicolumn{1}{r}{13.969} & \multicolumn{1}{r}{19.975}& \multicolumn{1}{r}{25.374} & \multicolumn{1}{r}{44.030}&\multicolumn{1}{r}{118.496}\\

        \multicolumn{1}{l}{280279} & \multicolumn{1}{l}{2972} & \multicolumn{1}{l|}{5960} &
		\multicolumn{1}{c}{2.26} & \multicolumn{1}{c}{1.38}& \multicolumn{1}{c}{0.94} & \multicolumn{1}{c}{0.56}&\multicolumn{1}{c|}{0.28}
		& \multicolumn{1}{r}{1.345} & \multicolumn{1}{r}{1.341}& \multicolumn{1}{r}{2.357} & \multicolumn{1}{r}{6.593}&\multicolumn{1}{r}{25.077}\\

        \multicolumn{1}{l}{65754} & \multicolumn{1}{l}{1202} & \multicolumn{1}{l|}{2400} &
		\multicolumn{1}{c}{3.39} & \multicolumn{1}{c}{1.93}& \multicolumn{1}{c}{0.91} & \multicolumn{1}{c}{0.49}&\multicolumn{1}{c|}{0.22}
		& \multicolumn{1}{r}{0.600} & \multicolumn{1}{r}{0.578}& \multicolumn{1}{r}{0.950} & \multicolumn{1}{r}{2.834}&\multicolumn{1}{r}{11.601}\\

        \multicolumn{1}{l}{80650} & \multicolumn{1}{l}{138769} & \multicolumn{1}{l|}{277546} &
		\multicolumn{1}{c}{3.28} & \multicolumn{1}{c}{1.65}& \multicolumn{1}{c}{0.85} & \multicolumn{1}{c}{0.49}&\multicolumn{1}{c|}{0.27}
		& \multicolumn{1}{r}{56.433} & \multicolumn{1}{r}{63.338}& \multicolumn{1}{r}{66.505} & \multicolumn{1}{r}{77.395}&\multicolumn{1}{r}{108.037}\\

        \multicolumn{1}{l}{1533028} & \multicolumn{1}{l}{49440} & \multicolumn{1}{l|}{98876} &
		\multicolumn{1}{c}{3.28} & \multicolumn{1}{c}{1.81}& \multicolumn{1}{c}{0.89} & \multicolumn{1}{c}{0.45}&\multicolumn{1}{c|}{0.22}
		& \multicolumn{1}{r}{16.416} & \multicolumn{1}{r}{23.538}& \multicolumn{1}{r}{27.837} & \multicolumn{1}{r}{43.133}&\multicolumn{1}{r}{104.672}\\  

		\multicolumn{1}{l}{49899} & \multicolumn{1}{l}{628} & \multicolumn{1}{l|}{1272} &
		\multicolumn{1}{c}{1.80} & \multicolumn{1}{c}{0.84}& \multicolumn{1}{c}{0.45} & \multicolumn{1}{c}{0.23}&\multicolumn{1}{c|}{0.12}
		& \multicolumn{1}{r}{0.477} & \multicolumn{1}{r}{1.019}& \multicolumn{1}{r}{3.994} & \multicolumn{1}{r}{18.218}&\multicolumn{1}{r}{82.120}\\
	
		\multicolumn{1}{l}{41141} & \multicolumn{1}{l}{19440} & \multicolumn{1}{l|}{39240} & \multicolumn{1}{c}{1.87} & \multicolumn{1}{c}{0.94}& \multicolumn{1}{c}{0.51} & \multicolumn{1}{c}{0.26}&\multicolumn{1}{c|}{0.13}
		& \multicolumn{1}{r}{7.301} & \multicolumn{1}{r}{10.421}& \multicolumn{1}{r}{14.600} & \multicolumn{1}{r}{29.337}&\multicolumn{1}{r}{88.769}\\
		
		\multicolumn{1}{l}{94884} & \multicolumn{1}{l}{23224} & \multicolumn{1}{l|}{47148} &
		\multicolumn{1}{c}{3.36} & \multicolumn{1}{c}{1.94}& \multicolumn{1}{c}{1.18} & \multicolumn{1}{c}{0.62}&\multicolumn{1}{c|}{0.29}
		& \multicolumn{1}{r}{8.293} & \multicolumn{1}{r}{12.069}& \multicolumn{1}{r}{15.321} & \multicolumn{1}{r}{34.692}&\multicolumn{1}{r}{124.510}\\
		
		\multicolumn{1}{l}{69220} & \multicolumn{1}{l}{22750} & \multicolumn{1}{l|}{45504} &
		\multicolumn{1}{c}{3.25} & \multicolumn{1}{c}{1.85}& \multicolumn{1}{c}{1.00} & \multicolumn{1}{c}{0.59}&\multicolumn{1}{c|}{0.36}
		& \multicolumn{1}{r}{8.872} & \multicolumn{1}{r}{10.532}& \multicolumn{1}{r}{15.278} & \multicolumn{1}{r}{26.975}&\multicolumn{1}{r}{69.279}\\
		
		\hline
	\end{tabular}
}
	% \label{table_MAP}
\end{table*}


